The Rapid Atmospheric Monitoring System of the Pierre Auger Observatory

The Pierre Auger Observatory is a facility built to detect air showers produced by cosmic rays above 10^17 eV. During clear nights with a low illuminated moon fraction, the UV fluorescence light produced by air showers is recorded by optical telescopes at the Observatory. To correct the observations for variations in atmospheric conditions, atmospheric monitoring is performed at regular intervals ranging from several minutes (for cloud identification) to several hours (for aerosol conditions) to several days (for vertical profiles of temperature, pressure, and humidity). In 2009, the monitoring program was upgraded to allow for additional targeted measurements of atmospheric conditions shortly after the detection of air showers of special interest, e.g., showers produced by very high-energy cosmic rays or showers with atypical longitudinal profiles. The former events are of particular importance for the determination of the energy scale of the Observatory, and the latter are characteristic of unusual air shower physics or exotic primary particle types. The purpose of targeted (or "rapid") monitoring is to improve the resolution of the atmospheric measurements for such events. In this paper, we report on the implementation of the rapid monitoring program and its current status. The rapid monitoring data have been analyzed and applied to the reconstruction of air showers of high interest, and indicate that the air fluorescence measurements affected by clouds and aerosols are effectively corrected using measurements from the regular atmospheric monitoring program. We find that the rapid monitoring program has potential for supporting dedicated physics analyses beyond the standard event reconstruction.

==> app_bts.tex <==
\begin{landscape}
\setlength{\topmargin}{-6mm}

\section{Appendix - \bts
\label{app:bts}}

\setlongtables
%\begin{longtable}{|r|r|r|r|r|l|l|}
\begin{longtable}{rrrrlll}
\hline
SMS~~~~~~~~~~~~~ & Launch~~~~~~~~~~~ & Launch & Event~~~~ & Event~~~ & ~~~~~~~Event & Comment \\ 
UTC time~~~~~~~~~ & UTC time~~~~~~~~~ & \#~~~ & GPS second & UTC time & ~~~~~~~~IDs & \\ 
\hline \hline \endhead
20 March 2009 - 02:15 & ---~~~~~~~~~~~~ & --- & 921548098 & --- & --- & problem with SMS \\ \hline
25 March 2009 - 05:45 & 25 March 2009 - 06:52 & 280 & 921993815 & --- & --- & problem with event data \\ \hline
28 March 2009 - 04:45 & ---~~~~~~~~~~~~  & --- & 922248208 & --- & --- & problem with SMS \\ \cline{1-1} \cline{4-7} 
28 March 2009 - 05:30  & & & 922251488 & --- & --- &  problem with SMS \\ \hline
03 April 2009 - 05:30 & 03 April 2009 - 06:22 & 281 & 922770424 & 05:06:49 & SD7525586 & \\
 & & & & & FD3/928/917 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD4/3038/1000 & reconstructed with all quality cuts, $E<2E19$  \\ \hline \hline
22 April 2009 - 08:00 & 22 April 2009 - 09:18 & 282 & 924421566 & 07:45:51 & SD7624453 &  \\
 & & & & & FD4/3066/5762 & reconstructed with all quality cuts \\
 & & & & & FD3/948/5706 & reconstructed with all quality cuts \\
 & & & & & FD2/2314/29100 & discarded \\ \hline
26 April 2009 - 08:45 & 26 April 2009 - 10:12 & 283 & 924769541 & 08:25:26 &SD7651722 &  \\
 & & & & & FD1/2785/7818 & reconstructed with all quality cuts \\
 & & & & & FD4/3073/6550 & discarded  \\ \hline
27 April 2009 - 03:00 & 27 April 2009 - 04:07 & 284 & 924835691 & 02:47:56 & SD7654632 &  \\
 & & & & & FD4/3074/2159 & reconstructed with all quality cuts, $E<2E19$  \\
 & & & & & FD3/963/2131 & reconstructed with all quality cuts, $E<2E19$  \\
 & & & & & FD2/2322/11412 & discarded  \\
 & & & & & FD1/2786/2238 & discarded \\ \hline
28 April 2009 - 07:15 & 28 April 2009 - 11:02 & 285 & 924937125 & 06:58:30 & SD7663682 & \\
 & & & & & FD1/2787/5662 & discarded  \\
 & & & & & FD2/2323/27112 & \\ \cline{1-1} \cline{4-7} 
28 April 2009 - 07:30 &  &  & 924937957 & 07:12:22 & SD7663796 & \multirow{2}{22pt}{discarded} \\
 & & & & & FD4/3075/5075 &  \\ \cline{1-1} \cline{4-7} 
28 April 2009 - 09:45 &  &  & 924945886 & 09:24:31 & SD7664874 &  \\
 & & & & & FD3/964/6448 & reconstructed with all quality cuts \\
 & & & & & FD4/3075/6763 & discarded  \\ \hline
30 April 2009 - 05:15 & 30 April 2009 - 06:42 & 286 & 925102731 & 04:58:36 & SD7676516 & \\
 & & & & & FD3/975/1266 & discarded  \\
 & & & & & FD2/2333/6702 & reconstructed with all quality cuts  \\ \cline{1-1} \cline{4-7} 
30 April 2009 - 07:45 & & & 925112002 & 07:33:07 & SD7677771 & \\
 & & & & & FD1/2800/4079 & reconstructed with all quality cuts \\
 & & & & & FD4/3086/3508 & discarded  \\ \hline
03 May 2009 - 08:00 & ---~~~~~~~~~~~~ & ---& 925371663 & --- & --- & no launch \\ \hline
03 May 2009 - 09:00 & ---~~~~~~~~~~~~ & ---& 925374977 & --- & --- & no launch \\ \hline \hline
23 May 2009 - 00:45 & 23 May 2009 - 02:17 & 287 & 927073684 & 00:27:49 & SD7745180 &\\
 & & & & & FD4/3104/719 & reconstructed with all quality cuts, $E<2E19$  \\
 & & & & & FD3/987/697 & reconstructed with all quality cuts \\ \cline{1-1} \cline{4-7} 
23 May 2009 - 04:15 & & & 927086106 & 03:54:51 & SD7747215 &  \\
 & & & & & FD4/3104/3034 & reconstructed with all quality cuts \\
 & & & & & FD3/987/3023 & reconstructed with all quality cuts \\ \hline \hline
17 June 2009 - 00:30 & 17 June 2009 - 02:27 & --- & 929233232 & --- & --- & unsuccessful launch \\ \hline
19 June 2009 - 03:15 & 19 June 2009 - 04:34 & --- & 929415777 & --- & --- & unsuccessful launch \\ \hline
20 June 2009 - 23:30 & 21 June 2009 - 00:40 & 288 & 929574608 & 23:09:53 & SD7868680 & \\
 & & & & & FD4/3135/128 & discarded \\
 & & & & & FD3/1010/148 & reconstructed with all quality cuts \\ \hline
21 June 2009 - 08:45 & ---~~~~~~~~~~~~ & --- & 929607601 & --- & --- & no launch \\ \hline
22 June 2009 - 08:45 & 22 June 2009 - 10:52 & 289 & 929694289 & 08:24:34 & SD7881162 &  \\
 & & & & & FD1/2883/84292 & reconstructed with all quality cuts \\
 & & & & & FD4/3136/7776 & discarded  \\ \cline{1-1} \cline{4-7} 
22 June 2009 - 10:15 & & & 929699895 & 09:58:00 & SD7882018 &  \multirow{4}{44pt}{discarded} \\
 & & & & & FD4/3136/9067 & \\
 & & & & & FD3/1013/564 & \\
 & & & & & FD1/2885/9218 & \\ \hline
23 June 2009 - 08:30 & 23 June 2009 - 10.55 & 290 & 929780099 & 08:14:44 & SD7889620 & \\
 & & & & & FD3/1015/4324 & reconstructed with all quality cuts \\
 & & & & & FD2/2402/603 & discarded \\ \hline
25 June 2009 - 08:45 & 25 June 2009 - 10:30 & 291 & 929953789 & 08:29:34 & SD7905339 & \\
 & & & & & FD2/2408/9032 & reconstructed with all quality cuts, $E<2E19$  \\ \hline
25 June 2009 - 23:45 & 26 June 2009 - 01:40 & 292 & 930007793 & 23:29:38 & SD7908207 &  \\
 & & & & & FD3/1020/210 & reconstructed with all quality cuts \\
 & & & & & FD4/3145/195 & discarded  \\ \hline
28 June 2009 - 04:45 & ---~~~~~~~~~~~~ & --- & 930198768 & --- & --- & no launch \\ \hline
29 June 2009 - 08:45 & 29 June 2009 - 09:50 & 293 & 930299418 & 08:30:03 & SD7929943 &  \\
 & & & & & FD4/3153/4852 & reconstructed with all quality cuts \\
 & & & & & FD3/1028/4822 & reconstructed with all quality cuts \\ \hline \hline
16 July 2009 - 06:45 & 16 July 2009 - 07:42 & 294 & 931759517 & 06:05:02 & SD7996239 & \\
 & & & & & FD1/2911/52 & discarded  \\
 & & & & & FD4/3163/53 & \\ \hline
23 July 2009 - 01:15 & 23 July 2009 - 01:44 & 295 & 932345558 & 00:52:23 & SD8043254 &  \\
 & & & & & FD4/3189/1775 & reconstructed with all quality cuts \\
 & & & & & FD2/2447/6555 & reconstructed with all quality cuts  \\ \cline{1-1} \cline{4-7} 
23 July 2009 - 04:45 & & & 932358922 & 04:35:07 & SD8045233 &  \\
 & & & & & FD4/3189/8154 & reconstructed with all quality cuts \\
 & & & & & FD2/2447/23750 & discarded  \\ \hline
25 July 2009 - 04:00 & 25 July 2009 - 04:47 & 296 & 932528217 & 03:36:42 & SD8060163 &  \\
 & & & & & FD1/2939/5486 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD2/2452/1435 & reconstructed with all quality cuts, $E<2E19$ \\ \cline{1-1} \cline{4-7} 
25 July 2009 - 04:30 & & & 932530725 & 04:18:30 & SD8060502 &  \multirow{2}{22pt}{discarded} \\
 & & & & & FD4/3192/5060 & \\ \hline
26 July 2009 - 05:45 & 26 July 2009 - 06:11 & 297 & 932621624 & 05:33:29 & SD8068317 & \\
 & & & & & FD4/3193/5457 & reconstructed with all quality cuts \\
 & & & & & FD3/1059/5083 & reconstructed with all quality cuts \\ \hline \hline
16 August 2009 - 08:15 & ---~~~~~~~~~~~~ & --- & 934444551 & --- & --- & \\ \cline{1-6}
17 August 2009 - 01:45 & ---~~~~~~~~~~~~ & --- & 934508159 & --- & --- & \\ \cline{1-6}
21 August 2009 - 06:00 & ---~~~~~~~~~~~~ & --- & 934868986 & --- & --- & \\ \cline{1-6}
22 August 2009 - 01:45 & ---~~~~~~~~~~~~ & --- & 934939533 & --- & --- & \\  \cline{1-1} \cline{4-6} 
22 August 2009 - 05:30 &  &  & 934952939 & --- & --- &  \\ \cline{1-1} \cline{4-6} 
22 August 2009 - 07:15 &  &  & 934959469 & --- & --- &  Software problems at BLS \\ \cline{1-6}
23 August 2009 - 00:15 & ---~~~~~~~~~~~~ & --- & 935021179 & --- & --- & \\ \cline{1-1} \cline{4-6} 
23 August 2009 - 05:00 & ---~~~~~~~~~~~~ & --- & 935037714 & --- & --- & \\ \cline{1-6}
24 August 2009 - 09:00 & ---~~~~~~~~~~~~ & --- & 935138740 & --- & --- & \\ \cline{1-6}
25 August 2009 - 03:30 & ---~~~~~~~~~~~~ & --- & 935205406 & --- & --- & \\ \cline{1-6}
26 August 2009 - 07:45 & ---~~~~~~~~~~~~ & --- & 935306542 & --- & --- & \\ \hline \hline
19 September 2009 - 01:45 & 19 September 2009 - 03:39 & 299 & 937359096 & 01:31:21 & SD8363936 & \\
 & & & & & FD4/3272/1338 & reconstructed with all quality cuts \\
 & & & & & FD3/1107/1311 & reconstructed with all quality cuts \\ \hline
20 September 2009 - 06:45 & ---~~~~~~~~~~~~ & --- & 937463190 & --- & --- &  no launch and \\
 & & & & & & for the rest of the FD shift no trigger - \\
 & & & & & & software problems with online reconstruction  \\ \hline \hline
13 October 2009 - 06:45 & 13 October 2009 - 08:12 & 300 & 939450622 & 06:30:07 & SD8497892 &  \multirow{2}{22pt}{discarded} \\
 & & & & & FD4/3299/4410 & \\ \hline
19 October 2009 - 03:45 & 19 October 2009 - 05:21 & 301 & 939958519 & 03:35:04 & SD8540459 &  \multirow{2}{22pt}{discarded} \\
 & & & & & FD3/1156/2712 & \\ \hline
21 October 2009 - 05:30 & 21 October 2009 - 07:30 & 302 & 940137263 & 05:14:08 & SD8557205 &  \\
 & & & & & FD2/2577/15684 & reconstructed with all quality cuts \\ \hline
22 October 2009 - 07:15 & 22 October 2009 - 08:47 & 303 & 940229493 & 06:51:18 & SD8565649 &  \\
 & & & & & FD4/3314/4494 & reconstructed with all quality cuts \\
 & & & & & FD1/3056/4269 & reconstructed with all quality cuts \\
 & & & & & FD3/1165/2655 & discarded  \\ \hline
23 October 2009 - 07:45 & ---~~~~~~~~~~~~ & ---& 940317999 & --- & --- & no launch \\ \hline
24 October 2009 - 05:00  & 24 October 2009 - 06:37 & 304 & 940394310 & 04:38:15 & SD8576896 & \\
 & & & & & FD1/3059/1184 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD4/3319/749 & reconstructed with all quality cuts , $E<2E19$\\ \hline \hline
14 November 2009 - 02:45 & ---~~~~~~~~~~~~ & --- & 942201199 & --- & --- & no launch \\ \hline
16 November 2009 - 06:15 & 16 November 2009 - 07:43 & 305 & 942386174 & 05:55:59 & SD8701300 &  \\
 & & & & & FD4/3350/4265 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD2/2607/18043 & reconstructed with all quality cuts \\ 
 & & & & & FD1/3083/4384 & reconstructed with all quality cuts \\
 & & & & & FD3/1196/421 & discarded \\ \hline
19 November 2009 - 07:30 & 19 November 2009 - 09:14 & 306 & 942649865 & 07:10:50 & SD8720247 &  \\
 & & & & & FD4/3355/303 & discarded \\ 
 & & & & & FD3/1200/4515 & reconstructed with all quality cuts, $E<2E19$ \\ \hline
20 November 2009 - 04:15 & 20 November 2009 - 05:52 & 307 & 942724785 & 03:59:30 & SD8725257  &  \\
 & & & & & FD4/3356/2668 & reconstructed with all quality cuts \\
 & & & & & FD3/1204/1533 & reconstructed with all quality cuts, $E<2E19$ \\ \hline
23 November 2009 - 07:45 & 23 November 2009 - 08:05 & 308 & 942992677 & 06:24:22 & SD8746845 &  \multirow{2}{22pt}{discarded} \\
 & & & & & FD4/3363/1029 &  \\ \hline \hline
11 December 2009 - 03:45 & 11 December 2009 - 05:20 & 309 & 944537481 & 03:31:06 & SD8830050 &  \\
 & & & & & FD3/1233/1653 & reconstructed with all quality cuts \\
 & & & & & FD2/2645/1914 & reconstructed with all quality cuts, $E<2E19$ \\ \hline
15 December 2009 - 04:45 & 15 December 2009 - 06:15 & 310 & 944886636 & 04:30:21 & SD8853685 &  \\
 & & & & & FD3/1241/2484 & reconstructed with all quality cuts \\
 & & & & & FD4/3391/2538 & reconstructed with all quality cuts \\ \hline
19 December 2009 - 01:00 & ---~~~~~~~~~~~~ & --- & 945229856 & --- & --- & problem with SMS \\ \hline \hline
19 January 2010 - 05:30 & ---~~~~~~~~~~~~ & --- & 947913207 & --- & --- & problem with SMS and \\
 & & & & & & for the rest of the FD shift no trigger - \\
 & & & & & & software problems with online reconstruction  \\ \hline \hline
07 February 2010 - 04:00 & ---~~~~~~~~~~~~ & --- & 949549739 &  --- & --- & no launch and \\
 & & & & & & for the rest of the FD shift no trigger - \\
 & & & & & & software problems with online reconstruction  \\ \hline \hline
14 March 2010 - 08:45 & 14 March 2010 - 10:22 & --- & 952590815 & --- & --- & unsuccessful launch \\ \hline
16 March 2010 - 02:00 & 16 March 2010 - 03:58 & 312 & 952738622 & 01:36:47 & SD9318812 &   \\
 & & & & & FD3/1316/559 & reconstructed with all quality cuts \\
 & & & & & FD2/2721/452 & reconstructed with all quality cuts \\ \cline{1-1} \cline{4-7}
16 March 2010 - 08:30 & & & 952762252 & 08:10:37 & SD9321462 &  \\
 & & & & & FD3/1316/9241 & reconstructed with all quality cuts \\
 & & & & & FD2/2721/10054 & reconstructed with all quality cuts, $E<2E19$ \\ \hline
19 March 2010 - 06:30 & ---~~~~~~~~~~~~ & --- & 953014558 & --- & --- & no launch \\ \hline \hline
14 April 2010 - 02:00 & 14 April 2010 - 03:25 & 313 & 955244979 & 01:49:24 & SD9452746 &   \\
 & & & & & FD4/3513/1747 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD2/2758/1764 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD1/3242/2082 & reconstructed with all quality cuts \\ \cline{1-1} \cline{4-7}
14 April 2010 - 04:15 & & & 955252567 & 03:55:52 & SD9453433 & \\
 & & & & & FD4/3513/3815 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD2/2758/3657 & discarded  \\ \hline \newpage
16 April 2010 - 06:30 & 16 April 2010 - 07:22 & 314 & 955433644 & 06:13:49 & SD9464726 &   \\
 & & & & & FD2/2762/7091 & reconstructed with all quality cuts \\
 & & & & & FD1/3244/8268 & reconstructed with all quality cuts \\
 & & & & & FD4/3521/7128 & discarded  \\ \hline
17 April 2010 - 05.00 & 17 April 2010 - 06:31 & 315 & 955514337 & 04:38:42 & SD9469504 &   \\
 & & & & & FD4/3523/3779 & reconstructed with all quality cuts \\
 & & & & & FD1/3245/5671 & reconstructed with all quality cuts \\
 & & & & & FD2/2763/4941 & discarded  \\ \cline{1-1} \cline{4-7}
17 April 2010 - 07:30 & & & 955523301 & 07:08:06 & SD9470374 &  \\
 & & & & & FD1/3245/9210 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD4/3523/6970 & discarded  \\ \hline \hline
10 May 2010 - 07:00 & 10 May 2010 - 08:07 & 316 & 957508744 & 06:38:49 & SD9569111 &  \\
 & & & & & FD4/3558/8099 & reconstructed with all quality cuts \\ \cline{1-1} \cline{4-7}
10 May 2010 - 09:00 & & & 957516063 & 08:40:48 & SD9569700 &   \\
 & & & & & FD2/2791/9987 & reconstructed with all quality cuts \\
 & & & & & FD4/3559/375 & reconstructed with all quality cuts \\ \cline{1-1} \cline{4-7}
10 May 2010 - 09:30 & & & 957518110 & 09:14:55 & SD9569838 &  \\
 & & & & & FD1/3271/456 & reconstructed with all quality cuts \\
 & & & & & FD4/3559/657 & reconstructed with all quality cuts \\
 & & & & & FD2/2791/10302 & discarded \\ \hline
12 May 2010 - 00:15 & 12 May 2010 - 01:15 & 317 & 957657539 & 23:58:44 & SD9578017 &  \\
 & & & & & FD2/2793/621 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD1/3275/453 & reconstructed with all quality cuts, $E<2E19$ \\ \hline
17 May 2010 - 23:30 & 18 May 2010 - 00:36 & 318 & 958173385 & 23:16:10 & SD9608800 &  \\
 & & & & & FD4/3571/60 & reconstructed with all quality cuts \\
 & & & & & FD2/2797/68 & reconstructed with all quality cuts \\ \hline
20 May 2010 - 06:20 & 20 May 2010 - 08:04 & 319 & 958371077 & 06:11:02 & SD9625601 & \multirow{2}{22pt}{discarded} \\
 & & & & & FD4/3579/5783 & \\ \cline{1-1} \cline{4-7}
20 May 2010 - 10:00 & & & 958384101 & 09:48:20 & SD9627281 &  \\
 & & & & & FD1/3287/6748 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD4/3579/8885 & reconstructed with all quality cuts, $E<2E19$ \\ \hline \newpage
21 May 2010 - 05:45 & 21 May 2010 - 07:01 & 320 & 958455264 & 05:34:09 & SD9630792 &  \\
 & & & & & FD4/3582/3214 & reconstructed with all quality cuts \\
 & & & & & FD1/3291/2654 & reconstructed with all quality cuts \\
 & & & & & FD3/1365/2363 & discarded \\ \hline \hline
16 June 2010 - 00:45 & ---~~~~~~~~~~~~ & ---& 960683560 & --- & --- & no launch \\ \hline \hline
8 July 2010 - 07:45 & 8 July 2010 - 09:50 & 321 & 962609683 & 07:34:28 & SD9868151 &  \\ 
 & & & & & FD4/3620/10249 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD3/1403/10037 & reconstructed with all quality cuts, $E<2E19$ \\ \hline
9 July 2010 - 03:30 & ---~~~~~~~~~~~~ & ---& 962680434 & --- & --- & no launch \\ \hline
11 July 2010 - 00:45 & 11 July 2010 - 02:10 & 322 & 962843774 & 00:35:59 & SD9894028 &  \\
 & & & & & FD1/3350/653 & reconstructed with all quality cuts \\
 & & & & & FD4/3625/1276 & discarded \\ \hline
12 July 2010 - 07:45 & ---~~~~~~~~~~~~ & ---& 962955337 & --- & --- & no launch \\ \hline \hline
6 August 2010 - 08:30 & ---~~~~~~~~~~~~ & ---& 965117610 & --- & --- & no launch \\ \hline
15 August 2010 - 02:45 & 15 August 2010 - 04:05 & 323 & 965874359 & 02:25:44 & SD10070294 & \\ 
 & & & & & FD2/2904/183 & discarded \\
 & & & & & FD3/1448/465 & discarded \\ \cline{1-1} \cline{4-7}
15 August 2010 - 05:30 & & & 965884638 & 05:17:03 & SD10071896 &  \\
 & & & & & FD4/3691/4369 & reconstructed with all quality cuts \\
 & & & & & FD3/1450/2447 & reconstructed with all quality cuts \\
 & & & & & FD2/2906/2253 & reconstructed with all quality cuts \\
 & & & & & FD1/3407/5490 & reconstructed with all quality cuts \\ \hline
19 August 2010 - 09:15 & 19 August 2010 - 11:05 & 324 & 966243498 & 08:58:03 & SD10097599 & \\ 
 & & & & & FD1/3410/1492 & discarded \\
 & & & & & FD2/2916/944 & reconstructed with all quality cuts, $E<2E19$ \\ \hline \hline
4 September 2010 - 02:30 & 4 September 2010 - 04:13 & 325 & 967601465 & 02:10:50 & SD10162229 &  \\
 & & & & & FD1/3411/2195 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD4/3700/1836 & reconstructed with all quality cuts, $E<2E19$ \\ \hline \hline
2 October 2010 - 02:45 & ---~~~~~~~~~~~~ & ---& 970021959 & --- & --- & no launch \\ \hline
2 October 2010 - 05:30 & ---~~~~~~~~~~~~ & ---& 970031362 & --- & --- & no launch \\ \hline \newpage
4 October 2010 - 07:30 & 4 October 2010 - 09:21 & 326 & 970211290 & 07:07:55 & SD10351057 & \\
 & & & & & FD4/3727/7546 & reconstructed with all quality cuts \\
 & & & & & FD1/3443/8889 & reconstructed with all quality cuts \\ \hline 
5 October 2010 - 02:15 & 5 October 2010 - 04:14 & 327 & 970278933 & 07:55:18 & SD10355445 & \\ 
 & & & & & FD1/3444/1330 & reconstructed with all quality cuts \\
 & & & & & FD2/2945/1148 & reconstructed with all quality cuts \\
 & & & & & FD4/3729/1162 & reconstructed with all quality cuts \\
 & & & & & FD3/1483/909 & discarded \\ \hline
7 October 2010 - 08:30 & 7 October 2010 - 10:18 & 328 & 970474772 & 08:19:17  & SD10375521  &  \\
 & & & & & FD4/3731/8749 & reconstructed with all quality cuts \\
 & & & & & FD1/3446/10065 & reconstructed with all quality cuts, $E<2E19$ \\ \hline
9 October 2010 - 04:45 & 9 October 2010 - 05:58 & 329 & 970633657 & 04:27:22 & SD10388800 & \\
 & & & & & FD4/3733/4359 & reconstructed with all quality cuts \\
 & & & & & FD3/1487/3920 & reconstructed with all quality cuts, $E<2E19$ \\ \hline
13 October 2010 - 07:30 & 13 October 2010 - 09:38 & 330 & 970989453 & 07:17:18 & SD10419862 & \\ 
 & & & & & FD4/3739/5277 & reconstructed with all quality cuts \\
 & & & & & FD3/1502/3961 & reconstructed with all quality cuts \\\hline \hline
31 October 2010 - 06:15 & ---~~~~~~~~~~~~ & ---& 972539796 & --- & --- & no launch \\ \hline
10 November 2010 - 07:45 & 10 November 2010 - 09:38 & 331 & 973408389 & 07:12:54  & SD10578064 & \\
 & & & & & FD1/3476/7662 & reconstructed with all quality cuts, $E<2E19$ \\
 & & & & & FD4/3767/6542 & reconstructed with all quality cuts \\
 & & & & & FD3/1531/4843 & discarded \\ \hline \hline
13 December 2010 - 07:30 & ---~~~~~~~~~~~~ & ---& 976259773 & --- & --- & no launch \\ \hline

\caption{Statistics of all SMS triggers, radio soundings, and related events since the beginning of the \bts 
program in March 2009. Horizontal double lines indicate new FD shifts.}
\end{longtable}
\end{landscape}


==> app_sts.tex <==
\section{Appendix - \sts
\label{app:sts}}
\setlength{\topmargin}{-12mm}

\setlongtables
\begin{longtable}{rrcccc}
	\hline
	GPS time & UTC time~~~~ & Los Leones & Los Morados & Loma Amarilla & Coihueco \\
	\hline \hline \endhead
	922770424 & 3/4/2009 - 05:06& - & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	922858437 & 4/4/2009 - 05:33& - & - & $\bullet$ & $\bullet$ \\
	%\hline
	924492057 & 23/4/2009 - 03:20& - & $\bullet$ & $\bullet$ & - \\
	%\hline
	924510528 & 23/4/2009 - 08:28& - & - & $\bullet$ & - \\
	%\hline
	924512002 & 23/4/2009 - 08:53& - & $\bullet$ & $\bullet$ & - \\
	%\hline
	924653103 & 25/4/2009 - 00:04& $\bullet$ & $\bullet$ & $\bullet$ & - \\
	%\hline
	924669599 & 25/4/2009 - 04:39& $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	924679672 & 25/4/2009 - 07:27& - & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	924763693 & 26/4/2009 - 06:48& - & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	924769541 & 26/4/2009 - 08:25& - & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	924835691 & 27/4/2009 - 02:47& $\bullet$ & $\bullet$ & - & $\bullet$ \\
	%\hline
	924844281 & 27/4/2009 - 05:11& $\bullet$ & - & $\bullet$ & $\bullet$ \\
	%\hline
	924850826 & 27/4/2009 - 07:00& - & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	924945886 & 28/4/2009 - 09:24& $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	925004377 & 29/4/2009 - 01:39& $\bullet$ & $\bullet$ & - & $\bullet$ \\
	%\hline
	925103072 & 30/4/2009 - 05:04& $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	925112002 & 30/4/2009 - 07:33& - & $\bullet$ & $\bullet$ & - \\
	%\hline
	925279464 & 2/5/2009 - 06:04& $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	925373121 & 3/5/2009 - 08:05& $\bullet$ & $\bullet$ & - & $\bullet$ \\
	%\hline
	926744246 & 19/5/2009 - 04:57& - & $\bullet$ & - & - \\
	%\hline
	926912754 & 21/5/2009 - 03:45& $\bullet$ & $\bullet$ & - & - \\
	%\hline
	926919170 & 21/5/2009 - 05:32& $\bullet$ & $\bullet$ & - & - \\
	%\hline
	926921087 & 21/5/2009 - 06:04& $\bullet$ & $\bullet$ & - & - \\
	%\hline
	926925037 & 21/5/2009 - 07:10& $\bullet$ & $\bullet$ & - & - \\
	%\hline
	926925530 & 21/5/2009 - 07:18& $\bullet$ & $\bullet$ & - & - \\
	%\hline
	927019796 & 22/5/2009 - 09:29& $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	927073684 & 23/5/2009 - 00:27& $\bullet$ & $\bullet$ & - & $\bullet$ \\
	%\hline
	927086106 & 23/5/2009 - 03:54& $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	929233232 & 17/6/2009 - 00:20& $\bullet$ & $\bullet$ & - & $\bullet$ \\
	%\hline
	929329900 & 18/6/2009 - 03:11& $\bullet$ & - & - & - \\
	%\hline
	929415777 & 19/6/2009 - 03:02& $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	929574608 & 20/6/2009 - 23:09& $\bullet$ & - & $\bullet$ & $\bullet$ \\
	%\hline
	929607601 & 21/6/2009 - 08:19& - & - & - & $\bullet$ \\
	%\hline
	930007793 & 25/6/2009 - 23:29& - & - & $\bullet$ & $\bullet$ \\
	%\hline
	931822230 & 16/7/2009 - 23:30& - & - & - & $\bullet$ \\
	%\hline
	932610393 & 26/7/2009 - 02:26& $\bullet$ & - & $\bullet$ & $\bullet$ \\
	%\hline
	934444551 & 16/8/2009 - 07:55& - & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	934508159 & 17/8/2009 - 01:35& $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	934952939 & 22/8/2009 - 05:08& $\bullet$ & $\bullet$ & - & $\bullet$ \\
	%\hline
	935021179 & 23/8/2009 - 00:06& $\bullet$ & $\bullet$ & - & $\bullet$ \\
	%\hline
	935037714 & 23/8/2009 - 04:41& $\bullet$ & $\bullet$ & - & $\bullet$ \\
	%\hline
	935138740 & 24/8/2009 - 08:45& - & $\bullet$ & - & - \\
	%\hline
	935205406 & 25/8/2009 - 03:16& - & - & - & $\bullet$ \\
	%\hline
	935314138 & 26/8/2009 - 09:28& $\bullet$ & $\bullet$ & - & $\bullet$ \\
	%\hline
	949549739 & 7/2/2010 - 03:48& - & - & $\bullet$ & - \\
	%\hline
	955252567 & 14/4/2010 - 03:55& - & $\bullet$ & - & - \\
	%\hline
	955433644 & 16/4/2010 - 06:13& - & $\bullet$ & $\bullet$ & - \\
	%\hline
	955523301 & 17/4/2010 - 07:08& - & $\bullet$ & - & - \\
	%\hline
	955782260 & 20/4/2010 - 07:04& - & $\bullet$ & - & - \\
	%\hline
	957516063 & 10/5/2010 - 08:40& - & - & - & $\bullet$ \\
	\hline
	957518110 & 10/5/2010 - 09:14& - & - & - & $\bullet$ \\
	%\hline
	957657539 & 11/5/2010 - 23:58& $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	958173385 & 17/5/2010 - 23:16& $\bullet$ & - & $\bullet$ & $\bullet$ \\
	%\hline
	958371077 & 20/5/2010 - 06:11& $\bullet$ & $\bullet$ & $\bullet$ & - \\
	%\hline
	958455264 & 21/5/2010 - 05:34& $\bullet$ & $\bullet$ & $\bullet$ & - \\
	%\hline
	960683560 & 16/6/2010 - 00:32& - & $\bullet$ & $\bullet$ & $\bullet$ \\
	%\hline
	962341872 & 5/7/2010 - 05:10& $\bullet$ & - & $\bullet$ & - \\
	%\hline
	962585024 & 8/7/2010 - 00:43& $\bullet$ & - & - & $\bullet$ \\
	%\hline
	962680434 & 9/7/2010 - 03:13& $\bullet$ & - & $\bullet$ & $\bullet$ \\
	%\hline
	962926721 & 11/7/2010 - 23:38& - & - & $\bullet$ & $\bullet$ \\
	%\hline
	962955337 & 12/7/2010 - 07:35& - & - & - & $\bullet$ \\
	\hline

\caption{List of executed \emph{Shoot-the-Shower} scans since April 2009.}
\label{table:sts}
\end{longtable}

